On the Modeling of Error Functions as High Dimensional Landscapes for Weight Initialization in Learning Networks

Next generation deep neural networks for classification hosted on embedded platforms will rely on fast, efficient, and accurate learning algorithms. Initialization of weights in learning networks has a great impact on the classification accuracy. In this paper we focus on deriving good initial weights by modeling the error function of a deep neural network as a high-dimensional landscape. We observe that due to the inherent complexity in its algebraic structure, such an error function may conform to general results of the statistics of large systems. To this end we apply some results from Random Matrix Theory to analyse these functions. We model the error function in terms of a Hamiltonian in N-dimensions and derive some theoretical results about its general behavior. These results are further used to make better initial guesses of weights for the learning algorithm.

==> conclusion.tex <==
\section {Conclusion}  \label{sec: conclusion}

Accurate classification is the goal of any multi-layer large neural network. Initialization of weights has a significant impact on the convergence of learning algorithms. We have provided a statistical method based on Random Matrix Theory for the weight initialization with probabilistic guarantees on the nature of minima reached in the high dimension landscape defined by the error function. Experimentally we have substantiated the novelty of our method in obtaining higher classification accuracy over well known initialization methods adopted by deep learning frameworks. 

